Stabilizing Linear Systems under Partial Observability: Sample Complexity and Fundamental Limits

We study the problem of stabilizing an unknown partially observable linear time-invariant (LTI) system. For fully observable systems, leveraging an unstable/stable subspace decomposition approach, state-of-art sample complexity is independent from system dimension $n$ and only scales with respect to the dimension of the unstable subspace. However, it remains open whether such sample complexity can be achieved for partially observable systems because such systems do not admit a uniquely identifiable unstable subspace. In this paper, we propose LTS-P, a novel technique that leverages compressed singular value decomposition (SVD) on the ''lifted'' Hankel matrix to estimate the unstable subsystem up to an unknown transformation. Then, we design a stabilizing controller that integrates a robust stabilizing controller for the unstable mode and a small-gain-type assumption on the stable subspace. We show that LTS-P stabilizes unknown partially observable LTI systems with state-of-the-art sample complexity that is dimension-free and only scales with the number of unstable modes, which significantly reduces data requirements for high-dimensional systems with many stable modes.

==> sections/archive.tex <==

\ziyi{Previous Proof}

\begin{proof}[Proof of \Cref{prop:analytic}]
 By \Cref{assumption:F_bnd}, there exists a controller $K(z)$ with $\delta_0>0$, such that for all $|z| \geq 1$, 
    \begin{align}
        &\delta_0 \leq \det(K(z)F_K(z)) = \det(K(z)(I-F(z)K(z))^{-1}) \notag
        \\
        \Rightarrow & \det(I-F(z)K(z)) \geq \frac{\delta_0}{\det(K(z))} 
        \label{eqn:delta0_det}
    \end{align}
    We then show there exists a controller $\hat{K}$ that is analytic on and outside of the unit cycle. From the derivation of \eqref{eqn:delta0_det}, we see that it suffice to show $\det(I-\hat{F}(z)K(z))>0$ for $z \in \mathbb{C}_{\geq 1}$.
    \begin{align}
        \det(I-\hat{F}(z)K(z)) &= \det(I - \hat{C}(zI-\hat{N}_1)^{-1}\hat{B}K(z)) \notag
    \\
    &= \det(I - \hat{C}\hat{S}(zI-\hat{S}^{-1}\hat{N}_1\hat{S})^{-1}\hat{S}^{-1}\hat{B}K(z))
    \label{eqn:det_inv1}
    \\
    &= \det(I - (zI-\hat{S}^{-1}\hat{N}_1\hat{S} )^{-1}\hat{S}^{-1}\hat{B}K(z)\hat{C}\hat{S})
    \label{eqn:det_inv2}
    \\
    &= \det(zI-\hat{S}^{-1}\hat{N}_1\hat{S} -\hat{S}^{-1}\hat{B}K(z)\hat{C}\hat{S})/\det(zI - \hat{S}^{-1}\hat{N}_1\hat{S}).
    \end{align}
    where we obtain \eqref{eqn:det_inv1} with $\det(I-A_1 A_2) = \det(I-A_2A_1)$ and \eqref{eqn:det_inv2} with $\det(I - A_1^{-1}A_2) = \det(A_1 - A_2)/\det(A_1)$. We can be sure that $\det(zI - \hat{S}^{-1}\hat{N}_1\hat{S}) > 0$ if we estimate $N_1$ with accuracy such that $\epsilon_N < |\lambda_k|-1$, or
    \begin{equation}
        \label{eqn:epsilon_req7}
        \frac{2\left(1+\zeta_{\epsilon_1}(N_1)(\lambda_1+\epsilon_1)\right)c_2\epsilon}{c_1 \sigma_{\min}(\tilde{\cO})} < |\lambda_k|-1 \quad \Rightarrow \quad \epsilon \leq \frac{c_1 \sigma_{\min}(\tilde{\cO})}{2\left(1+\zeta_{\epsilon_1}(N_1)(\lambda_1+\epsilon_1)\right)c_2}(|\lambda_k|-1).
    \end{equation}
    Therefore, we can guarantee the following inequality holds
    \begin{equation}
        \det(zI-\hat{S}^{-1}\hat{N}_1\hat{S} -\hat{S}^{-1}\hat{B}K(z)\hat{C}\hat{S}) > \frac{\delta_0 \det(zI - \hat{S}^{-1}\hat{N}_1\hat{S})}{\det(K(z))} 
    \end{equation}
    \ziyi{previous part}
    The controller $\hat{K}(z)$ is designed such that $\hat{K}(z)\hat{F}_{\hat{K}}(z)$ is analytic on and outside of the unit cycle. Therefore, 
\begin{align*}
    \hat{K}(z) \hat{F}_{\hat{K}}(z) = & \hat{K}(z) (I-\hat{F}(z)\hat{K}(z))^{-1}.
\end{align*}
may only have pole inside the unit disc, i.e. there exists $\delta_1 \neq 0$, such that
\begin{equation}
\label{eqn:det_hat_F}
    \det(I-\hat{F}(z)\hat{K}(z)) = \delta_1.
\end{equation}
Similarly, it suffices to prove that 
\begin{equation}
    \label{eqn:del_F}
    \det(I - F(z)\hat{K}(z)) \neq 0.
\end{equation}
To that end, we can further expand \eqref{eqn:det_hat_F} as follows:
\begin{align*}
    \det(I - \hat{F}(z)\hat{K}(z)) &= \det(I - \hat{C}(zI-\hat{N}_1)^{-1}\hat{B}\hat{K}(z))
    \\
    &= \det(I - \hat{C}\hat{S}(zI-\hat{S}^{-1}\hat{N}_1\hat{S})^{-1}\hat{S}^{-1}\hat{B}\hat{K}(z))
    \\
    &= \det(I - (zI-\hat{S}^{-1}\hat{N}_1\hat{S} )^{-1}\hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S})
    \\
    &= \det(zI-\hat{S}^{-1}\hat{N}_1\hat{S} -\hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S})/\det(zI - \hat{S}^{-1}\hat{N}_1\hat{S}).
\end{align*}
where we obtain the second equality with $\det(I-AB) = \det(I-BA)$ and the third equality by $\det(I - A^{-1}B) = \det(A - B)/\det(A)$. 
%\guannan{missing a ``$-$'' in the third equality. }
Therefore, for any $\norm{z}\geq 1$, there exists $\delta_2 \neq 0$, such that
\begin{equation*}
    \det(zI- \hat{S}^{-1}\hat{N}_1\hat{S} -\hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S}) \geq \delta_2.
\end{equation*}
Similarly, it suffices to prove that 
\begin{equation*}
    \det(zI - N_1 - R_1B \hat{K}(z)CQ_1) \neq 0.
\end{equation*}
We can bound the gap between $zI - N_1 - R_1B \hat{K}(z)CQ_1$ and $zI-\hat{S}^{-1}\hat{N}_1 \hat{S} - \hat{B}\hat{K}(z)\hat{C}$ as follows:
\begin{align*}
    &\norm{(zI-\hat{N}_1 -\hat{B}\hat{K}(z)\hat{C}) - (zI - N_1 - R_1B \hat{K}(z)CQ_1)} 
    \\
    =&\norm{(zI-\hat{S}^{-1}\hat{N}_1\hat{S} -\hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S}) - (zI - N_1 - R_1B \hat{K}(z)CQ_1)} 
    \\
    =& \norm{N_1 - \hat{S}^{-1}\hat{N}_1 \hat{S} + R_1B \hat{K}(z)CQ_1 - \hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S}}
    \\
    \leq & \norm{N_1 - \hat{S}^{-1}\hat{N}_1 \hat{S}} + \norm{R_1B \hat{K}(z)CQ_1 - \hat{S}^{-1}\hat{B}\hat{K}(z)CQ_1 +\hat{S}^{-1}\hat{B}\hat{K}(z)CQ_1 - \hat{S}^{-1}\hat{B}\hat{K}(z)\hat{C}\hat{S}}
    \\
    \leq & \norm{N_1 - \hat{S}^{-1}\hat{N}_1 \hat{S}} + \norm{R_1 B - \hat{S}^{-1}\hat{B}}\norm{\hat{K}(z)CQ_1} + \norm{CQ_1 - \hat{C}\hat{S}}\norm{\hat{B}\hat{K}(z)}
    \\
    \leq & \epsilon_N + \epsilon_B\norm{K(z)CQ_1} + \epsilon_C \norm{\hat{B}\hat{K}(z)}.
\end{align*}

Therefore, when picking $\epsilon_N, \epsilon_B, \epsilon_C$ as in the problem statement, we can guarantee that $\det(zI - N_1 R_1B \hat{K}(z)CQ_1) \neq 0$.
\end{proof}

==> sections/conclusion.tex <==
In this paper, we examined the necessary and sufficient conditions for the stabilization of a partially observable LTI system and proposed a novel SVD-based robust controller design framework. Future work includes studying the transfer function from the process noise $w_t$ to $y_t$, and improving the complexity bound in \Cref{thm:main}. 
